Wrong Prediction, Right Answer: Recovering Evidence from Collapsed LLM Sequence Scores

When a large language model fails a reasoning task, it is often assumed to lack the underlying capability. However, this conflates a genuine absence of reasoning with a late-stage output bottleneck. We observe a consistent readout gap across diverse reasoning benchmarks: hidden-state probes successfully decode correct answers even when native sequence scoring completely collapses due to structural biases. To test whether instance-specific logic survives this collapse, we introduce a diagnostic protocol using a minimal, target-label-free additive correction. Fitting just two parameters on as few as 25 unlabeled examples recovers 9--34 accuracy points for Qwen3.5 models, transferring successfully to OLMo-2-1B and Llama-3.1-8B. Crucially, these recovered decisions persist on hard instances unresolved by simple lexical overlap and significantly exceed count-preserving permutation baselines. Our results show that many apparent zero-shot reasoning deficits are expression failures masking intact internal logic, urging a narrower interpretation of benchmark evaluations.

==> tables/proofwriter_native_prior_mean_robustness.tex <==
% Auto-generated from ProofWriter mean-normalized native prior-calibration summaries.
% Regenerate with: bash scripts/run_proofwriter_native_prior_mean_calibration.sh && bash scripts/run_proofwriter_native_prior_mean_permutation_null.sh && bash scripts/run_proofwriter_native_prior_mean_bow_stratified.sh && bash scripts/run_proofwriter_native_prior_mean_sensitivity.sh && python scripts/render_paper_tables.py --table proofwriter_native_prior_mean_robustness
\begin{tabular}{lccccc}
\toprule
Audit & $N$ & Raw Acc. & Cal./Min Acc. & $\Delta$ / Obs.-Null & Macro-F1 \\
\midrule
Mean sequence, OOD & 1000 & 0.333 & 0.653 [0.623, 0.682] & +0.320 [+0.274, +0.366] & 0.650 \\
Prediction-count null & 1000 & 0.333 & 0.653 & +0.320 ($p=0.0001$) & 0.650 \\
TF-IDF-missed stratum & 576 & 0.366 & 0.627 & +0.294 ($p=0.0001$) & 0.627 \\
$\pm 0.10$ prior sensitivity & 1000 & 0.333 & 0.611 / 0.651 & +0.278 worst & 0.594 min \\
\bottomrule
\end{tabular}

